Improving hp-Variational Physics-Informed Neural Networks for Steady-State Convection-Dominated Problems

This paper proposes and studies two extensions of applying hp-variational physics-informed neural networks, more precisely the FastVPINNs framework, to convection-dominated convection-diffusion-reaction problems. First, a term in the spirit of a SUPG stabilization is included in the loss functional and a network architecture is proposed that predicts spatially varying stabilization parameters. Having observed that the selection of the indicator function in hard-constrained Dirichlet boundary conditions has a big impact on the accuracy of the computed solutions, the second novelty is the proposal of a network architecture that learns good parameters for a class of indicator functions. Numerical studies show that both proposals lead to noticeably more accurate results than approaches that can be found in the literature.

==> sections/Loss_functions/Crosswind+L2.tex <==
\subsubsection{Crosswind loss functional + L2 weight regularization loss}

Similar to our approach with SUPG, we incorporate L2 regularization in conjunction with Crosswind Loss functional to enhance the model's generalization and prevent overfitting. This combined approach is crucial in scenarios where maintaining accuracy in the presence of sharp gradients or discontinuities is essential.
The Crosswind  Loss function + $L^2$ weight regularization loss functional is defined by 
\begin{equation}
    \mathcal L_{\alpha, \lambda}^{\mathrm{cw}} = \mathcal{L}^{\text{hard}}_{\text{var}} + \alpha\frac{|\Omega|}{N_{1}}\sum_{i=1}^{N_1} \phi\left(|\bb^{\perp}(\bx_{i})\cdot \nabla u(\bx_{i})|\right) + \frac{\lambda}{N}\sum_jw_j^2.
\end{equation}


==> sections/Loss_functions/Crosswind.tex <==
\subsubsection{Crosswind loss functional}

Based on the observation that spurious oscillations in SUPG finite element solutions are connected
with large derivatives in crosswind direction, it was proposed in \cite{john2011posteriori} to 
penalize crosswind derivatives. A functional with such a penalization was also included in the numerical 
studies in \cite{FHJ24}.

The definition of the crosswind loss uses the weighting function 
$\phi:\mathbb{R}\to\mathbb{R}$ defined by 
\begin{equation}
    \phi(x) = 
    \begin{cases}
        \sqrt{x},\quad &\text{if } x\geq 1 \\ 
        0.5(5x^2-3x^3)\quad &\text{else}
    \end{cases}
\end{equation}
In two dimension, for any $x\in\Omega$, a vector in crosswind direction (orthogonal to the convection field) 
is given by 
\begin{equation}
    \bb^{\perp}(\bx) = 
    \begin{cases}
        \dfrac{(b_2(\bx),-b_1(\bx))}{\|\bb\|_2},\quad &\text{if } \bb(\bx)\neq\mathbf{0}, \\  
        \mathbf{0},\quad &\text{else}
    \end{cases}
\end{equation}
where $\bb = (b_1,b_2)^T$ and $\|\cdot\|_2$ is the Euclidean norm of the vector. Then the crosswind loss 
functional is defined by 
\begin{equation}
    \mathcal L_{\alpha}^{\mathrm{cw}} = \mathcal{L}^{\text{hard}}_{\text{var}} + \alpha\frac{|\Omega|}{N_{1}}\sum_{i=1}^{N_1} \phi\left(|\bb^{\perp}(\bx_{i})\cdot \nabla u(\bx_{i})|\right),
\end{equation}
where $|\Omega|$ is the measure of $\Omega$, $N_1$ is the number of quadrature points in the domain, and
$\alpha$ is a hyperparameter that needs to be tuned.

==> sections/Loss_functions/SUPG+L2.tex <==
c\subsection{SUPG stabilization loss + $L^2$ weight regularization loss}
The SUPG method ensures that the solution remains stable and accurate, especially in the presence of strong convection effects. The $L^2$ regularization further aids by penalizing large parameter values, thereby preventing overfitting and enhancing the model's ability to generalize   

By integrating SUPG with $L^2$ regularization, we achieve a robust and stable model capable of accurately capturing complex phenomena in convection-dominated problems while maintaining generalization through regularization.

\begin{equation*}
    \mathcal{L}_{\mathcal{SUPG}, \lambda}
 = \int_{\Omega} \tau(\bx)\left(\bb\cdot\nabla u(\bx) + cu(\bx)-f(\bx)\right)\left(\bb\cdot\nabla v(\bx)\right)\ \mathrm{d}\bx + \frac{\lambda}{N}\sum_jw_j^2, 
\end{equation*}
 
Then, the SUPG stabilization + $L^2$ weight regularization loss functional is given by 
\begin{equation}
    \mathcal{L}^{\mathcal{SUPG}}_{\tau, \lambda} = \mathcal{L}^{\text{hard}}_{\text{var}} + \mathcal{L}_{\mathcal{SUPG}, \lambda}
    \label{Eq: Supg_L2_loss}
\end{equation}
where $\mathcal{L}^{\text{hard}}_{\text{var}}$ is the variational loss defined in  \eqref{eq:vpinn_hard_loss}.


==> sections/Methodology/methodology.tex <==
\subsection{Existing implementation of hp-VPINNs}

Consider the two-dimensional Poisson equation in $\Omega \subseteq \mathbb{R}^2$.  
\begin{align}
    \begin{split}
        -\nabla^2 u(\mathbf{x}) &= f(\mathbf{x}), \quad \ \mathbf{x} \in \Omega\\
     u(\mathbf{x}) &= 0, \quad \qquad \mathbf{x} \in \partial\Omega 
    \end{split}
    \label{eqn:poisson2D}
\end{align}
The variational physics-informed neural networks~(VPINNs) methodology takes advantage of the variational form of the Partial Differential Equation~(PDE) to calculate the loss function integral to the model optimization process. Given the complexities associated with symbolic integration of all terms, VPINNs utilize numerical quadrature techniques, such as Gauss-Lobatto or Gauss-Legendre quadrature, for the integral evaluation. The variational form of the PDE can be computed as follows.
Let $H_1(\Omega)$ be the standard Sobolev space denoted by $V$, which is defined by

\[
 H^1_0(\Omega):=\left\{v \in \text{\textit{H}}^1(\Omega) : v = 0 \quad \text{on} \quad \partial \Omega \right\}.
\]
Now, we can derive the variational form of Equation~\ref{eqn:poisson2D} by multiplying it by the test function $v \in V$, and integrating it over the domain $\Omega$. The variational form of the Poisson equation reads

\[
a(u,v) = f(v) \quad \text {for all } v \in V, 
\]
where, 
\begin{align}
    \begin{split}
        a(u,v) &:= \int_{\Omega} \nabla u \cdot \nabla v \; d \Omega, \quad \qquad \; \text{for all } v \in V\\
        f(v) &:= \int_{\Omega} fv \; d \Omega,\quad \quad  \quad \qquad \text{for all } v \in V
    \end{split}
    \label{eq:poisson2D_weakform_general}
\end{align}
The term $a(u,v)$ is obtained by multiplying the test function $v$ with the Laplacian operator and using integration by parts to transfer one derivative to v; refer~(\cite{ganesan2017finite}) for more details. This variational form of~\eqref{eqn:poisson2D} serves as a component of the loss function, combined with the boundary loss as shown in Equation~(\ref{eqn:vpinns_final_loss_fn_abbr}). Algorithm~(1) in appendix effectively outlines the steps for calculating the VPINN training loss, following the methodology in the hp-VPINNs GitHub repository (\cite{hp_vpinns_github}). The algorithm iteratively evaluates each cell in the computational domain to compute the local PDE loss. This approach requires gradients and test function values to be sourced from predefined basis functions, whereas the neural network provides solution variables and their gradients at specific quadrature points. Following this, the algorithm sums up the losses from all cells and merges them with the supervised boundary loss, detailed in Equation~\eqref{eqn:VPINNs_Bound_Loss}. This comprehensive loss function is then utilized in neural network training, ensures the VPINNs adherence to both the physics of the PDE and its boundary conditions.






\subsection*{Need for Efficient Implementation of hp-VPINNs}
While hp-VPINNs present an advantageous approach to mitigating the spectral bias commonly observed in neural network solutions for high-frequency phenomena, their computational efficiency poses significant challenges. The training time of hp-VPINNs exhibits a nonlinear increase with increasing number of computational cells, as shown in Figure~\ref{fig:pinn_vs_fastvpinn_time}(a,b). This increase in computational demand for training time makes the method less feasible for applications that involve a large number of cells. Furthermore, the current implementation, as outlined in the hp-VPINNs framework, is restricted to structured meshes, in particular structured quadrilateral elements. This limitation stems from the fact that for such elementary geometric configurations, the transformation of derivatives from the reference cell to the actual domain can be efficiently achieved by a simple multiplication with a constant Jacobian factor for each cell. In contrast, practical applications often necessitate the analysis of unstructured mesh within complex domains, which requires transformations, such as bilinear transformations, to accurately map the gradients from the reference cell to the actual domain. This added complexity in handling non-structured meshes is a crucial consideration for the broader applicability and effectiveness of hp-VPINNs in solving practical problems.



\subsection*{Improvement to existing hp-VPINNs}

Several optimizations were required to improve the existing hp-vpinns algorithm and develop the final FastVPINNs algorithm. The advantages and challenges associated with each optimization are outlined below.
\newline \textit{Note :~}Starting here, the variable \texttt{N\_test} denotes the number of test functions present in the specified cell, \texttt{N\_quad} represents the number of quadrature points in the given cell and finally \texttt{N\_cells} indicates the total number of cells in the current domain. \texttt{jac} denotes the Jacobian of the cell. \texttt{jac\_x} and \texttt{jac\_y} denotes the Jacobian of the cell in x-direction and in y-direction respectfully.

\subsubsection*{Precomputation of intermediate shape function values}
Analysis of Algorithm~(1) reveals a computational pattern dominated by recurring multiplicative operations linked to shape function derivatives and quadrature weights, which will be constant throughout epochs. Consequently, there is no computational necessity to repetitively calculate these values in every training iteration.
Furthermore, for the calculation of \texttt{ Diff\_x}, the iterative process employed in Algorithm~(1) can be efficiently reformulated as a matrix vector operation. In this optimized representation, the premultiplier matrix \texttt{A} of dimension \texttt{N\_test x N\_quad}, contains the values of the shape function multiplied by the corresponding quadrature weights. The gradient of the solution, as computed by the neural network, is encapsulated within the vector \texttt{u\_sol\_nn\_grad\_x}, exhibiting a dimensionality of \texttt{N\_quad x 1}. This matrix-vector paradigm not only simplifies the computation, but also potentially enhances the algorithm's computational efficiency by leveraging the inherent advantages of BLAS operations within the GPU.  This pre-computation strategy eliminates the need for repeated calculations that involve shape functions and gradients with quadrature weights, leading to substantial computational savings. Algorithm~(2) outlines the procedure for assembling the premultiplier matrices and the loss computation using the same.

\subsubsection*{Eliminating Cell Looping}
Even with the elimination of redundant calculations and the incorporation of matrix vector operations to enhance efficiency, the algorithm still necessitates iterating through the number of cells in domain. Consequently, it performs forward passes N\_cells times to compute the solution and backward passes N\_cells times to determine the gradients of the solution. However, in the case of uniformly refined mesh structures, the Jacobian transformation remains constant for all points within each cell. This consistency is also observed in meshes with parallel edges (as shown in Figure~\ref{fig:meshes}), where the jacobian is the same for all test functions at any given set of quadrature points. The only variation in these matrix vector computations within each cell loop is the \texttt{jac/jac\_x}, which is multiplied by the neural network solution and its gradients and can differ for each cell. Therefore, we can store these jacobians (which transfer the reference gradients to the actual gradients) for each cell in a vector of size \texttt{N\_quad x 1}. These vectors can then be stacked to create a matrix of size \texttt{N\_quad x N\_cells}, as shown in Algorithm~(3). We first arrange the input quadrature points for all cells with a shape of \texttt{N\_quad * N\_cells, <Num\_Of\_Input\_Dimension>}. We then feed these points into the neural network to obtain the solution and its gradients. These gradients are then reshaped to \texttt{N\_quad x N\_cells}. Next, we perform an element-wise multiplication between this matrix and the premultiplier\_jacobian matrix. The resulting matrix is then multiplied by the precomputed shape function gradient matrices using matrix-matrix multiplication to calculate the integral of the term over the domain. Since the element-wise operation includes the multiplication of the Jacobian of a specific cell (arranged in columns) with the corresponding solution gradients, this operation handles the transformation of gradients from the actual domain to the reference domain when multiplied with the shape function matrices. By strategically pre-computing and rearranging the computations, we can compute the integral term in a single matrix-matrix multiplication operation. One advantage of this approach is that it completely eliminates the need for looping through cells, which in turn reduces the number of backpropagation steps performed by the neural network in each epoch. This optimization is the main factor that contributes to the improved performance of the algorithm. The pseudocode of the algorithm is provided in Algorithm~(3).


\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth, height=0.5\textheight, keepaspectratio]{images/meshes.png}
    \caption{quad meshes with cells having constant jacobian}
    \label{fig:meshes}
\end{figure}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     Optimisattion - 3 - Fast VPINNs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection*{FastVPINNs : Tensor-based framework generalizable for complex geometries}

Although the above optimized version of the code is significantly faster, it relies on the assumption that the Jacobian remains constant for a given reference-to-original transformation within each cell. However, in complex geometries with skewed quad elements, the Jacobian can vary at each quadrature point and for every shape function due to bilinear transformation. Consequently, we cannot create a premultiplier Jacobian of size \texttt{ N\_quad} x 1 that can accurately account for the transformation of gradients from the reference domain to the actual domain when multiplied with the precomputed shape function/gradient matrices. This results in us having a different premultiplier matrices for each cell, which again results in a cell looping algorithm similar to Algorithm~(1). The presence of this constraint renders this optimization impractical for complex geometry problems in real-world scenarios. 

In this paper, we present a novel approach to stack the premultiplier matrices along the third dimension, creating a tensor of shape \texttt{N\_cells x N\_test x N\_quad}, and stack the solution vectors to form a 2D matrix of size \texttt{N\_quad x N\_cells}. This allows for specific tensor-based operations, where each 2D slice of the tensor along the N\_cell dimension is multiplied with the corresponding column of the solution matrix, resulting in a vector of size \texttt{N\_test x 1} that fills the corresponding column of the output vector. Due to the current configuration of the input tensors and output matrices, it is not possible to directly obtain the cell-wise residuals by using straight forward blas routines. However, by transposing the solution gradients to have dimensions of \texttt{N\_cells x N\_quad} instead of \texttt{N\_quad x N\_cells}, we can use tensorflow's \texttt{tf.linalg.matvec} to perform tensor-matrix multiplication. This will result in a solution of dimensions \texttt{N\_cells x N\_test}. To obtain the desired output dimension of \texttt{N\_test x N\_cells}, we simply need to transpose this matrix. This approach based on tensors enables us to efficiently manage complex meshes with a large number of cells, all without the requirement of looping through each cell. Moreover, it enables us to effectively utilize the tensor-cores present in the GPU, thereby further improving the execution speed of this algorithm.


\newline

\textit{ Please note that in the subsequent sections of this paper, we will use the term 'FastVPINN' algorithm to refer to the generalized tensor-based approach described in Algorithm (4).}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\textwidth, height=0.5\textheight, keepaspectratio]{images/fastvpinns.png}
    \caption{Fast-Vpinns tensor schematic}
    \label{fig:fast_vpinns}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     ALGORITHM - 4 VPINNS Optimisation 3.0 in Listing fomat
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\rule{\textwidth}{1pt}  % Line before the listing
Algorithm 4: Generalised Tensor-based FastVPINNs Algorithm \newline
\noindent\rule{\textwidth}{1pt}  % Line before the listing
\begin{lstlisting}[language=Python, label={lst:algorithm_3}]
# Compute the prematrix multipliers for shapefunctions and gradients 
# in actual cell for all domains and stack them into 3D tensor. 
# Shape: N_cell x N_test x N_quad
shape_val_mat_tensor = tf.stack(shape_val_mat_list, axis=0)
grad_x_mat_tensor = tf.stack(grad_x_mat_list, axis=0)
grad_y_mat_tensor = tf.stack(grad_y_mat_list, axis=0)

# Compute Forcing Matrix
for n in range(num_cells):
    for j in range(num_test_functions):
        #integral for int(f.v) is already computed and stored in force_fn
        force_matrix[n][j] = jac[n][q] * force_fn[n][j] * quad_wt[q] * shape_funtion_val[j][q]

# Stack the quadrature points for each cell. 
for cell in range(n_cells):
    quad_points_in_domain.stack(quad_input[cell])

def train_step():
    # obtain solution for the quadrature points in entire domain
    sol = model(quad_points_in_domain)

    
    # obtain gradients
    u_sol_nn_grad_x, u_sol_nn_grad_y = model.get_gradients() 

    # reshape gradients to get matrix (N_quad * N_cells)
    u_sol_nn_grad_x = u_sol_nn_grad_x.reshape(N_cells, N_quad)
    u_sol_nn_grad_y = u_sol_nn_grad_y.reshape(N_cells, N_quad)

    # Perform a tensor-matrix operation between shape grad and nn sol grad 
    # to evaluate the integral int(du/dx. dv.dx) and int(du/dy. dv.dy)
    # Resulting matrix shape will be N_test * N_cells
    diff_x = tf.transpose(tf.linalg.matvec(grad_x_mat_tensor, u_sol_nn_grad_x))
    diff_y = tf.transpose(tf.linalg.matvec(grad_y_mat_tensor, u_sol_nn_grad_y))

    # Subract the forcing matrix from diff to get residual 
    residual_matrix = diff_x + diff_y - force_matrix 

    # obtain mse error for each cell
    residual_cells =  reduce_mean(square(residual_matrix), axis=0)

    # sum all residuals of cells
    variational_loss = reduce_sum(residual_cells)

    # get dirichlet loss
    dirichlet_loss = reduce_mean(square(actual - model.predict(dirichlet_input)))

    # Final loss ( Beta is a hyper parameter)
    final_loss = variational_loss + beta * dirichlet_loss

    optimiser.step()

    

\end{lstlisting}
\noindent\rule{\textwidth}{1pt}  % Line before the listing





==> sections/Numerical_studies_1/Mixed_boundary.tex <==
% \subsection{Solution with mixed boundary layers}
\subsubsection*{Problem-3: Solution with mixed boundary layers  (P3)}\label{sec:mixed}
This example is proposed in \cite{JOHN20081997}. The data for problem 
\eqref{eq:cdr_eqn} are given by 
$\Omega = (0,1)^2$, $\epsilon = 10^{-8}$, $\bb = (1,0)^T$, $c = 0$.



Instead of using an analytical solution, we employ a simulated solution obtained through the MUAS (Monotone Upwind-type Algebraically Stabilized) method. The MUAS method, formulated in \cite{DBLP:journals/corr/abs-2111-08697}, is designed to handle the challenges of solving convection-diffusion equations, strongly effective in scenarios involving high Péclet numbers, where traditional numerical methods may suffer from issues such as spurious oscillations or excessive numerical diffusion.
% and the prescribed solution has the form \cite{yadav2023artificial} 
% \begin{align}
%     \begin{split}
%         u(x,y):= &\alpha x + \frac{(R-L-\alpha)(e^{(-\beta(1-x))}-e^{-\beta})}{1-e^{-\beta}} + L   \\ 
%         \text{where}\quad&\alpha = \frac{f}{b_1},\;\beta = \frac{b_1}{\varepsilon},\;L = 0,\; R=0.
%     \end{split}
%     \label{eq:Mixed_layer}
% \end{align}


Homogenous Dirichlet condition of solution is imposed at boundary. The solution possesses two types of boundary layers : one exponential layer at $x=1$ and two parabolic boundary layers at $y=0$ and $y=1$.  
Figure~\ref{fig:exact_P}(c) shows the exact solution.
% given in \eqref{eq:Mixed_layer}.
\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{images/results/Result_exact.png}
    \caption{Exact solution for (a) Circular interior layer (b) Outflow layer (c) Mixed boundary layers problem}
    \label{fig:exact_P}
\end{figure}

==> sections/Numerical_studies_1/Modified_ansatz.tex <==
\subsection{Experimentation with adaptive stabilization parameter}

To address this, we modified our indicator function to account for the convective field by incorporating sharp gradients aligned with the direction of convection. Specifically, we introduced two distinct indicator functions: $h_1$ for outflow boundary layer problem \eqref{eq:Outflow_layer} and $h_2$ for mixed boundary layer problem \eqref{eq:Mixed_layer}. These modified indicator functions are designed to better capture the directional behavior of the solution, thereby improving the accuracy of our predictions. 
\begin{equation}
    \begin{split}
        &h_1(x,y) = (1 - e^{-k_1 x})(1 - e^{-k_1 y})(1-e^{-k_2(1 - x)})(1-e^{-k_2(1 - y)}), \\
        &h_2(x,y) = (1 - e^{-k_1 x})(1 - e^{-k_2 y})(1-e^{-k_2(1 - x)})(1-e^{-k_2(1 - y)}), \\
        \text{with}\quad &k_1 = 30,\;\quad k_2 = 10/\varepsilon
    \end{split}
    \label{Eq: Modified_ansatz_out}
\end{equation}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.99\textwidth]{images/results/Modified_ansatz/Modified_Ansatz.png}
    \caption{(a) $h_1(x,y)$, (b) $h_2(x,y)$}
    \label{fig:Modified_ansatz}
\end{figure}
We have seen from earlier set of experiments that including $\mathcal{L}_{\text{SUPG}}$ (given in \eqref{eqn:SUPG_Loss}) in the loss functional has improved the accuracy of predicted solution. Initially, we employed a constant stabilization parameter $\tau$, but this approach had limitations in adapting to varying problem complexities. In our current work, we have advanced this approach by incorporating a neural network to dynamically learn the stabilization parameter $\tau$. This adaptation allows the model to adjust $\tau$ based on the specific features of the problem, further refining the accuracy and robustness of the solution predictions. We are modelling $\tau(x)$ in the following way :
\begin{equation}
    \tau(x) = \tau_g. \tilde\tau(x)  
\end{equation} 
where $\tau_g$ termed as $\tau$ growth, controlling the strength of the stabilization factor ($\tau$) and $\tilde\tau:\Omega\to\mathbb R$ which captures the spatial variation of $\tau$. \\ 
The VPINN archiitecture has two output nodes : one for predicting the solution of PDE and other for predicting $\tilde\tau$. $\tau_g$ is the hyperparameter that needs to be fine tuned. $\tau$ is then used in the calculation of $\mathcal{L}_{\tau}^{\text{SUPG}}$ (given in \eqref{Eq: Supg_loss} for training the neural network.   \\
In this new set of experiments, all the configuration of network remains same as discussed in \ref{subsec:Initial Experimentation}, except that the output layer of network has two nodes. for the best resulting hyperparameter, the experiments has been conducted 10 times with random seed to check the robustness of the method.  



\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.3}
% \resizebox{1\textwidth}{!}{
    \begin{tabular}{|l|c|c|}
    \hline
    \textbf{Loss functional} & \textbf{$L_2$ error} & \textbf{$L_{inf}$ error} \\ 
    \hline
    $\mathcal{L}^{\text{hard}}_{\text{var}}$ & $1.69 \times 10^{-4}$ & $8.18 \times 10^{-4}$ \\ 
    \hline
    $\mathcal{L^{SUPG}_\tau}$ ; $\tau_g = 1$ & $1.03 \times 10^{-4}$ & $4.65 \times 10^{-4}$  \\
    \hline
    % PDE Loss ; $\tau_g = 0.1$ & $1.35 \times 10^{-4}$ & $7.04 \times 10^{-5}$ & $6.22 \times 10^{-4}$ & $2.18 \times 10^{-4}$ \\ \hline
    % PDE Loss ;  $\tau_g = 0.05$ & $1.42 \times 10^{-4}$ & $2.88 \times 10^{-5}$ & $6.49 \times 10^{-4}$ & $1.48 \times 10^{-4}$ \\ \hline
    \end{tabular}
% }
\caption{Outflow Layer - modified indicator function with PDE loss and adaptive stabilization parameter}
\label{tab:loss_functionals}
\end{table}


\begin{figure}[h!]
    \centering
\includegraphics[width=0.99\textwidth]{images/results/Modified_ansatz/Outflow_tau_0_l2_0.png}
    \caption{Results for $P1$ with $\mathcal{L}^{\text{hard}}_{\text{var}}$ (a) Predicted Solution, (b) Pointwise Absolute Error} 
    \label{fig:Modified_ansatz_solution}
\end{figure}



\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.3}
% \resizebox{1\textwidth}{!}{
    \begin{tabular}{|l|c|c|}
    \hline
    \textbf{Loss functional} & \textbf{$L_2$ error}  & \textbf{$L_{inf}$ error} \\ 
    \hline
    $\mathcal{L}^{\text{hard}}_{\text{var}}$  & $8.31 \times 10^{-4}$ & $2.10 \times 10^{-3}$  \\
    \hline
    $\mathcal{L^{SUPG}_\tau}$ ; $\tau_g = 1$ & $9.41 \times 10^{-4}$ & $2.87 \times 10^{-3}$ \\   
    \hline
    % PDE Loss ; $\tau_g = 0.1$ & $1.36 \times 10^{-2}$ & $4.67 \times 10^{-6}$ & $5.43 \times 10^{-1}$ & $2.39 \times 10^{-4}$ \\ \hline
    % PDE Loss ; $\tau_g = 0.01$ & $1.36 \times 10^{-2}$ & $5.72 \times 10^{-6}$ & $5.43 \times 10^{-1}$ & $2.10 \times 10^{-4}$ \\ \hline
    % PDE Loss ; $\tau_g = 0.001$ & $1.36 \times 10^{-2}$ & $9.15 \times 10^{-6}$ & $5.43 \times 10^{-1}$ & $3.65 \times 10^{-4}$ \\ \hline
    \end{tabular}
% }
\caption{Mixed boundary Layer - modified indicator function with PDE loss and adaptive stabilization parameter}
\label{tab:loss_functionals_second}
\end{table}


\begin{figure}[h!]
    \centering
\includegraphics[width=0.99\textwidth]{images/results/Modified_ansatz/Sangeeta_tau_0_l2_0.png}
    \caption{Results for $P3$ with $\mathcal{L}^{\text{hard}}_{\text{var}}$ (a) Predicted Solution, (b) Pointwise Absolute Error} 
    \label{fig:Modified_ansatz_solution}
\end{figure}





==> sections/Numerical_studies_2/Mixed_boundary.tex <==
% \subsection{Solution with mixed boundary layers}
\subsubsection*{Problem-3: Solution with mixed boundary layers  (P3)}\label{sec:mixed}
This example is proposed in \cite{JOHN20081997}. The data for problem 
\eqref{eq:cdr_eqn} are given by 
$\Omega = (0,1)^2$, $\epsilon = 10^{-8}$, $\bb = (1,0)^T$, $c = 0, f=1$. \\

Instead of using an analytical solution, we employ a simulated solution obtained through the MUAS (Monotone Upwind-type Algebraically Stabilized) method. The MUAS method, formulated in \cite{DBLP:journals/corr/abs-2111-08697}, is designed to handle the challenges of solving convection-diffusion equations, strongly effective in scenarios involving high Péclet numbers, where traditional numerical methods may suffer from issues such as spurious oscillations or excessive numerical diffusion.
% and the prescribed solution has the form \cite{yadav2023artificial} 
% \begin{align}
%     \begin{split}
%         u(x,y):= &\alpha x + \frac{(R-L-\alpha)(e^{(-\beta(1-x))}-e^{-\beta})}{1-e^{-\beta}} + L   \\ 
%         \text{where}\quad&\alpha = \frac{f}{b_1},\;\beta = \frac{b_1}{\varepsilon},\;L = 0,\; R=0.
%     \end{split}
%     \label{eq:Mixed_layer}
% \end{align}


Homogenous Dirichlet condition of solution is imposed at boundary.   
Figure~\ref{fig:exact_Sang} shows the exact solution.
% given in \eqref{eq:Mixed_layer}.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.99\textwidth]{images/results/Result_exact.png}
%     \caption{Exact solution for (a) Circular interior layer (b) Outflow layer (c) Mixed boundary layers problem}
%     \label{fig:exact_P}
% \end{figure}


==> sections/Preliminaries/cdr_equations.tex <==

\subsection{Convection-dominated CDR equation}
The CDR equation \eqref{eq:cdr_eqn} is said to be convection dominated when
\begin{equation*}
    \varepsilon \ll L||\bb||,
\end{equation*}
where $L$ is the characteristic length of the domain and $||\bb|| = \sqrt{b_1^2+b_2^2}$ is the magnitude of convective field. With the Péclet number, $Pe$, defined as 
\begin{equation*}
    Pe = \frac{L||\bb||}{\varepsilon},
\end{equation*}
the convection-dominated regime can also be characterized by $Pe \gg 1$.



==> sections/Preliminaries/hard_constraint.tex <==

\subsection{Convection-dominated CDR equation}
The CDR equation \eqref{eq:cdr_eqn} is said to be convection dominated when
\begin{equation*}
    \varepsilon \ll L||\bb||,
\end{equation*}
where $L$ is the characteristic length of the domain and $||\bb|| = \sqrt{b_1^2+b_2^2}$ is the magnitude of convective field. With the Péclet number, $Pe$, defined as 
\begin{equation*}
    Pe = \frac{L||\bb||}{\varepsilon},
\end{equation*}
the convection-dominated regime can also be characterized by $Pe \gg 1$.



==> sections/Preliminaries/pinn.tex <==
\subsection{Physics-Informed Neural Networks}
A deep neural network is a parametric function of $x$, which we denote by $u_{\text{NN}}(x; \theta_W, \theta_b)$, where $\theta_W$ and $\theta_b$ are the weights and biases of the network, respectively. A neural network consisting of $h$ hidden layers, with the $i^{\text{th}}$ layer containing $n_i$ neurons, can be represented mathematically as:
\begin{equation*}
   u_{\text{NN}}(x; \theta_W, \theta_b) = l \circ \mathrm{T}^{(h)} \circ \mathrm{T}^{(h-1)} \hdots \circ \mathrm{T}^1(x).
    \label{eq:NN}
\end{equation*}
Here, $l : \mathbb{R}^{n_h} \rightarrow \mathbb{R}$ is a linear mapping in the output layer and $\mathrm{T}^{(i)}(\cdot) = \sigma(\theta_W^{(i)} \times \cdot + \theta_b^{(i)})$ is a non-linear mapping in the $i^{th}$ layer $( i= 1, 2, \cdots , h)$, with the non-linear activation function $\sigma$ and the weights $\theta_W^{(i)}$ and biases $\theta_b^{(i)}$ of the respective layers.

By training the neural network, we can approximate the solution of \eqref{eq:cdr_eqn} with the neural network's output $u_{\text{NN}}(x; \theta_W, \theta_b)$. PINNs systematically reduce the residual arising from the governing equations specified in equation~\eqref{eq:cdr_eqn} to achieve the estimation $u_{\text{NN}}(x; \theta_W, \theta_b)$. Specifically, the residual related to the PDE, which we denote by $\mathcal{P}$, can be defined as:
\begin{equation}
        \mathcal{P}(x; \theta_W, \theta_b) =  -\varepsilon\Delta u_{\text{NN}} + \mathbf{b}\cdot\nabla u_{\text{NN}} + c u_{\text{NN}} -f, \quad \ \text{in}  \ \  \Omega.
\end{equation}
This residual is computed at $N_T$ training points within the domain to find the difference between the expected solution and the neural network's predictions. In particular, we define the PDE loss as 
\begin{equation}
    \mathcal{L}_p(\theta_W,\theta_b) = \frac{1}{N_T}\sum_{t=1}^{N_T}\left|\mathcal{P}(x_t;\theta_W,\theta_b)\right|^2.
\end{equation}
\subsubsection{Enforcing boundary constraints in PINNs}
To ensure that the network learns a unique solution while satisfying the PDE, we have to apply the boundary condition as mentioned in \eqref{eq:cdr_eqn}. The boundary condition can be enforced strictly by using the neural network output as part of a solution ansatz that satisfies the boundary condition (\cite{lu2021physics}).
\begin{equation}
    u^{\text{hard}}_{\text{NN}}(x; \theta_W, \theta_b) = j(x) + h(x)u_{\text{NN}}(x; \theta_W, \theta_b).
    \label{eq:hard_ansatz}
\end{equation}
Here, $j(x)$ is a continuous function in $\Omega$ that satisfies $j(x)=g(x)$ for $x \in \partial\Omega$ and $h(x)$ is a function satisfying 
\begin{equation*}
    h(x)= 
    \begin{cases}
      0, & x \in \partial\Omega, \\
      > 0, & \text{elsewhere.}
    \end{cases}
\end{equation*}
We can now define a PDE residual, $ \mathcal{P}^{\text{hard}}$ and its corresponding loss $\mathcal{L}^{\text{hard}}_{\text{PINN}}$:
\begin{align}
    \begin{split}
        \mathcal{P}^{\text{hard}}(x; \theta_W, \theta_b) &=  -\varepsilon\Delta u^{\text{hard}}_{\text{NN}} + \mathbf{b}\cdot\nabla u^{\text{hard}}_{\text{NN}} + c u^{\text{hard}}_{\text{NN}} -f, \quad \ \text{in}  \ \  \Omega, \\
        \mathcal{L}^{\text{hard}}_{\text{PINN}}(\theta_W,\theta_b) &= \frac{1}{N_T}\sum_{t=1}^{N_T}\left|\mathcal{P^{\text{hard}}}(x_t;\theta_W,\theta_b)\right|^2.
    \end{split}
    \label{eqn:hard_loss}
\end{align}

Another way to apply the boundary condition is to simply add a boundary loss by defining a boundary residual and summing it up across points sampled on the boundary, as shown below.
\begin{align}
    \begin{split}
        \mathcal{B}(x; \theta_W, \theta_b) &= u_{\text{NN}}(x; \theta_W, \theta_b) - g(x), \quad \ \text{in}  \ \  \Omega, \\
        \mathcal{L}_b(\theta_W,\theta_b) &= \frac{1}{N_D}\sum_{d=1}^{N_D}\left|\mathcal{B}(x_d;\theta_W,\theta_b)\right|^2.
    \end{split}
    \label{eqn:soft_loss}
\end{align}
In the case of soft boundary constraints, the network is trained on a total loss comprising of the PDE loss and boundary loss, where the latter is usually multiplied with some scaling factor $\tau$ to control the penalty on the boundary term.
\begin{equation}
    \mathcal{L}^{\text{soft}}_{\text{PINN}}(\theta_W,\theta_b) = \mathcal{L}_p + \tau\mathcal{L}_b.
\end{equation}
